Keep Various Trajectories: Promoting Exploration of Ensemble Policies in Continuous Control

The combination of deep reinforcement learning (DRL) with ensemble methods has been proved to be highly effective in addressing complex sequential decision-making problems. This success can be primarily attributed to the utilization of multiple models, which enhances both the robustness of the policy and the accuracy of value function estimation. However, there has been limited analysis of the empirical success of current ensemble RL methods thus far. Our new analysis reveals that the sample efficiency of previous ensemble DRL algorithms may be limited by sub-policies that are not as diverse as they could be. Motivated by these findings, our study introduces a new ensemble RL algorithm, termed \textbf{T}rajectories-awar\textbf{E} \textbf{E}nsemble exploratio\textbf{N} (TEEN). The primary goal of TEEN is to maximize the expected return while promoting more diverse trajectories. Through extensive experiments, we demonstrate that TEEN not only enhances the sample diversity of the ensemble policy compared to using sub-policies alone but also improves the performance over ensemble RL algorithms. On average, TEEN outperforms the baseline ensemble DRL algorithms by 41\% in performance on the tested representative environments.

==> sections/Rebuttal.tex <==
\setcounter{section}{0}
\setcounter{equation}{0}
\setcounter{figure}{0}
\renewcommand\thesection{\Alph{section}}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\textwidth]{Images/results_plot_sup.pdf}
    \caption{Learning curves for 5 continuous control tasks on DMControl suite. For better visualization, the curves are smoothed uniformly. The bolded line represents the average evaluation over 10 seeds. The shaded region represents the standard deviation of the average evaluation over 10 seeds.}
    \label{fig:dmc}
\end{figure}

\begin{figure}[H]
    \centering
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \subfigure{
        \includegraphics[width=1\linewidth]
        {Images/bias_cheetah.pdf}
        }

        \subfigure{
            \includegraphics[width=1\linewidth]{Images/bias_hopper.pdf}
        }
        \setcounter{subfigure}{0}
        \subfigure[Performance]{
            \includegraphics[width=1\linewidth]{Images/bias_walker.pdf}
            
        }
    \end{minipage}
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \subfigure{
            \includegraphics[width=0.93\linewidth]{Images/bias_cheetah2.pdf}
        }
        
        \subfigure{
            \includegraphics[width=0.99\linewidth]{Images/bias_hopper2.pdf}
        }
        \setcounter{subfigure}{1}
        \subfigure[Average Bias]{
            \includegraphics[width=0.99\linewidth]{Images/bias_walker2.pdf}
        }
    \end{minipage}
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \subfigure{
            \includegraphics[width=1\linewidth]{Images/bias_cheetah3.pdf}
        }

        \subfigure{
            \includegraphics[width=1\linewidth]{Images/bias_hopper3.pdf}
        }
        \setcounter{subfigure}{2}
        \subfigure[Performance]{
            \includegraphics[width=1\linewidth]{Images/bias_walker3.pdf}
        }
    \end{minipage}
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \subfigure{
            \includegraphics[width=0.93\linewidth]{Images/bias_cheetah4.pdf}
        }

        \subfigure{
            \includegraphics[width=0.99\linewidth]{Images/bias_hopper4.pdf}
        }
        \setcounter{subfigure}{3}
        \subfigure[Average Bias]{
            \includegraphics[width=0.99\linewidth]{Images/bias_walker4.pdf}
        }
    \end{minipage}
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \subfigure{
            \includegraphics[width=1\linewidth]{Images/alpha_cheetah.pdf}
        }

        \subfigure{
            \includegraphics[width=1\linewidth]{Images/alpha_hopper.pdf}
            
        }
        \setcounter{subfigure}{4}
        \subfigure[Performance]{
            \includegraphics[width=1\linewidth]{Images/alpha_walker.pdf}
        }
    \end{minipage}
    
\caption{TEEN ablation results for MuJoCo environments (From top to bottom are HalfCheetah-v3, Hopper-v3, Walker2d-v3.). The first column shows the effect of ensemble size $N$ on performance. The second column shows the effect of ensemble size $N$ on estimation bias. The third and fourth columns show the effect of target value number $M$ on both performance and estimation bias respectively. The fifth column shows the effect of weight parameter $\alpha$ on performance.}
\label{fig::ablation}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.35\linewidth]{Images/Humanoid-v3.pdf}
    \caption{Learning curves for MuJoCo complex task Humanoid-v3. For better visualization,the curves are smoothed uniformly. The bolded line represents the average evaluation over 5 seeds. The shaded region represents a standard deviation of the average evaluation over 5 seeds.}
    \label{fig:enter-label}
\end{figure}

